ProNeRF: Learning Efficient Projection-Aware Ray Sampling for Fine-Grained Implicit Neural Radiance Fields

Recent advances in neural rendering have shown that, albeit slow, implicit compact models can learn a scene's geometries and view-dependent appearances from multiple views. To maintain such a small memory footprint but achieve faster inference times, recent works have adopted `sampler' networks that adaptively sample a small subset of points along each ray in the implicit neural radiance fields. Although these methods achieve up to a 10$\times$ reduction in rendering time, they still suffer from considerable quality degradation compared to the vanilla NeRF. In contrast, we propose ProNeRF, which provides an optimal trade-off between memory footprint (similar to NeRF), speed (faster than HyperReel), and quality (better than K-Planes). ProNeRF is equipped with a novel projection-aware sampling (PAS) network together with a new training strategy for ray exploration and exploitation, allowing for efficient fine-grained particle sampling. Our ProNeRF yields state-of-the-art metrics, being 15-23x faster with 0.65dB higher PSNR than NeRF and yielding 0.95dB higher PSNR than the best published sampler-based method, HyperReel. Our exploration and exploitation training strategy allows ProNeRF to learn the full scenes' color and density distributions while also learning efficient ray sampling focused on the highest-density regions. We provide extensive experimental results that support the effectiveness of our method on the widely adopted forward-facing and 360 datasets, LLFF and Blender, respectively.

==> Figures/figure_ablation_network.tex <==
\begin{tblr}{
  stretch = 0,
  colsep  = 0pt,
  colspec = {Q[h,c]Q[h,c]},
  rowsep = 0.3pt,
}
  \small{Ground Truth} & \small{EpiNeRF-12 (25.17dB)} \\ 
  \includegraphics[width=88mm]{Figures/figure_ablation_network/fern_gt.jpg} &\includegraphics[width=88mm]{Figures/figure_ablation_network/fern_our.jpg}\\
  \includegraphics[width=88mm]{Figures/figure_ablation_network/fern_gt_2.jpg} &\includegraphics[width=88mm]{Figures/figure_ablation_network/fern_our_2.jpg}\\
  \vspace{2mm}&\vspace{2mm}\\
  \small{W/o $\sigma$ shift (24.20dB)} & \small{W/o auxiliary loss (24.26dB)}\\
  \includegraphics[width=88mm]{Figures/figure_ablation_network/fern_no_add.jpg} &\includegraphics[width=88mm]{Figures/figure_ablation_network/fern_no_aux.jpg}\\
    \includegraphics[width=88mm]{Figures/figure_ablation_network/fern_no_add_2.jpg} &\includegraphics[width=88mm]{Figures/figure_ablation_network/fern_no_aux_2.jpg}\\
\end{tblr}

==> Figures/figure_ablation_network_2.tex <==
\begin{tblr}{
  stretch = 0,
  colsep  = 0pt,
  colspec = {Q[h,c]Q[h,c]},
  rowsep = 0.3pt,
}
  \small{Ground Truth} & \small{EpiNeRF-12 (25.17dB)} \\
  \includegraphics[width=88mm]{Figures/figure_ablation_network_2/fern_gt.jpg} &\includegraphics[width=88mm]{Figures/figure_ablation_network_2/fern_our.jpg}\\
  \includegraphics[width=88mm]{Figures/figure_ablation_network_2/fern_gt_2.jpg} &\includegraphics[width=88mm]{Figures/figure_ablation_network_2/fern_our_2.jpg}\\
\vspace{2mm}&\vspace{2mm}\\
  \small{W/o point offsets (24.31dB)} & \small{W/o affine $\alpha$ (24.69dB)}\\
  \includegraphics[width=88mm]{Figures/figure_ablation_network_2/fern_no_offset.jpg} &\includegraphics[width=88mm]{Figures/figure_ablation_network_2/fern_no_affine.jpg}\\
    \includegraphics[width=88mm]{Figures/figure_ablation_network_2/fern_no_offset_2.jpg} &\includegraphics[width=88mm]{Figures/figure_ablation_network_2/fern_no_affine_2.jpg}\\
\end{tblr}

==> Figures/figure_ablation_network_3.tex <==
\begin{tblr}{
  stretch = 0,
  colsep  = 0pt,
  colspec = {Q[h,c]Q[h,c]},
  rowsep = 0.3pt,
}
  \small{Ground Truth} & \small{EpiNeRF-12 (25.17dB)} \\
  \includegraphics[width=88mm]{Figures/figure_ablation_network_4/fern_gt.jpg} &\includegraphics[width=88mm]{Figures/figure_ablation_network_4/fern_our.jpg}\\
  \includegraphics[width=88mm]{Figures/figure_ablation_network_4/fern_gt_2.jpg} &\includegraphics[width=88mm]{Figures/figure_ablation_network_4/fern_our_2.jpg}\\
\vspace{2mm}&\vspace{2mm}\\
  \small{W/o point offsets (24.31dB)} & \small{W/o auxiliary loss $\alpha$ (24.26dB)}\\
  \includegraphics[width=88mm]{Figures/figure_ablation_network_4/fern_no_offset.jpg} &\includegraphics[width=88mm]{Figures/figure_ablation_network_4/fern_no_aux.jpg}\\
    \includegraphics[width=88mm]{Figures/figure_ablation_network_4/fern_no_offset_2.jpg} &\includegraphics[width=88mm]{Figures/figure_ablation_network_4/fern_no_aux_2.jpg}\\
\end{tblr}

==> Figures/figure_ablation_network_4.tex <==
\begin{tblr}{
  stretch = 0,
  colsep  = 15pt,
  colspec = {Q[h,c]Q[h,c]},
  rowsep = 0.3pt,
}
  \small{Ground Truth} & \small{ProNeRF-12 (25.17dB)} \\
  \includegraphics[width=62mm]{Figures/figure_ablation_network_4/fern_gt.jpg} &\includegraphics[width=62mm]{Figures/figure_ablation_network_4/fern_our.jpg}\\
  \includegraphics[width=62mm]{Figures/figure_ablation_network_4/fern_gt_2.jpg} &\includegraphics[width=62mm]{Figures/figure_ablation_network_4/fern_our_2.jpg}\\
\vspace{2mm}&\vspace{2mm}\\
  \small{W/o point offsets (24.31dB)} & \small{W/o auxiliary loss $l_a$ (24.26dB)}\\
  \includegraphics[width=62mm]{Figures/figure_ablation_network_4/fern_no_offset.jpg} &\includegraphics[width=62mm]{Figures/figure_ablation_network_4/fern_no_aux.jpg}\\
    \includegraphics[width=62mm]{Figures/figure_ablation_network_4/fern_no_offset_2.jpg} &\includegraphics[width=62mm]{Figures/figure_ablation_network_4/fern_no_aux_2.jpg}\\
\end{tblr}

==> Figures/figure_ablation_training_strat.tex <==
\begin{tblr}{
  stretch = 0,
  colsep  = 15pt,
  colspec = {Q[h,c]Q[h,c]},
  rowsep = 0.3pt,
}
  \small{Ground Truth} & \small{ProNeRF-12 (25.17dB)} \\
  \includegraphics[width=62mm]{Figures/figure_ablation_training/fern_gt.jpg} &\includegraphics[width=62mm]{Figures/figure_ablation_training/fern_our.jpg}\\
  \includegraphics[width=62mm]{Figures/figure_ablation_training/fern_gt_2.jpg} &\includegraphics[width=62mm]{Figures/figure_ablation_training/fern_our_2.jpg}\\
  \vspace{2mm}&\vspace{2mm}\\
  
  \small{Without exploration (24.00dB)} & \small{Without exploitation (24.31dB)}\\
  \includegraphics[width=62mm]{Figures/figure_ablation_training/fern_only_finetune.jpg} &\includegraphics[width=62mm]{Figures/figure_ablation_training/fern_only_sampler.jpg}\\
    \includegraphics[width=62mm]{Figures/figure_ablation_training/fern_only_finetune_2.jpg} &\includegraphics[width=62mm]{Figures/figure_ablation_training/fern_only_sampler_2.jpg}\\
\end{tblr}

==> Figures/figure_blender.tex <==
\begin{tblr}{
  stretch = 0,
  colsep  = 0pt,
  colspec = {Q[h,c]Q[h,c]Q[h,c]},
  rowsep = 0.3pt,
}
  \small{Ground Truth} & \small{ProNeRF-32 Prune} & \small{TensoRF-CP (ECCV 2022)}\\
  \includegraphics[width=60mm]{Figures/figure_blender/chair_gt.jpg} &\includegraphics[width=60mm]{Figures/figure_blender/chair_our.jpg}&\includegraphics[width=60mm]{Figures/figure_blender/chair_tensorf.jpg} \\
  \includegraphics[width=60mm]{Figures/figure_blender/ficus_gt.jpg} &\includegraphics[width=60mm]{Figures/figure_blender/ficus_our.jpg}&\includegraphics[width=60mm]{Figures/figure_blender/ficus_tensorf.jpg} \\
  \includegraphics[width=60mm]{Figures/figure_blender/hotdog_gt.jpg} &\includegraphics[width=60mm]{Figures/figure_blender/hotdog_our.jpg}&\includegraphics[width=60mm]{Figures/figure_blender/hotdog_tensorf.jpg} \\
  \includegraphics[width=60mm]{Figures/figure_blender/materials_gt.jpg} &\includegraphics[width=60mm]{Figures/figure_blender/materials_our.jpg}&\includegraphics[width=60mm]{Figures/figure_blender/materials_tensorf.jpg} \\
  \includegraphics[width=60mm]{Figures/figure_blender/ship_gt.jpg} &\includegraphics[width=60mm]{Figures/figure_blender/ship_our.jpg}&\includegraphics[width=60mm]{Figures/figure_blender/ship_tensorf.jpg} \\
\end{tblr}

==> Figures/figure_donerf.tex <==
\begin{tblr}{
  stretch = 0,
  colsep  = 0pt,
  colspec = {Q[h,c]Q[h,c]Q[h,c]},
  rowsep = 0.3pt,
}
  \small{Ground Truth} & \small{Our EpiNeRF} & \small{DONeRF \cite{donerf}} \\
  \includegraphics[width=58.5mm]{Figures/figure_donerf/sanmiguel_gt.jpg} &\includegraphics[width=58.5mm]{Figures/figure_donerf/sanmiguel_our.jpg}&\includegraphics[width=58.5mm]{Figures/figure_donerf/sanmiguel_donerf.jpg}\\
  \includegraphics[width=58.5mm]{Figures/figure_donerf/forest_gt.jpg} &\includegraphics[width=58.5mm]{Figures/figure_donerf/forest_our.jpg}&\includegraphics[width=58.5mm]{Figures/figure_donerf/forest_donerf.jpg}\\
  \includegraphics[width=58.5mm]{Figures/figure_donerf/pavillon_gt.jpg} &\includegraphics[width=58.5mm]{Figures/figure_donerf/pavillon_our.jpg}&\includegraphics[width=58.5mm]{Figures/figure_donerf/pavillon_donerf.jpg}\\

\end{tblr}

==> Figures/figure_inter_results.tex <==
\begin{tblr}{
  stretch = 0,
  colsep  = 0pt,
  colspec = {Q[h,c]Q[h,c]Q[h,c]Q[h,c]Q[h,c]Q[h,c]Q[h,c]},
  rowsep = 0.3pt
}
    $C_{s0}$ & $C_{s1}$ & $C_{s1}$ (no shader) & $\hat{C}$ (Full EpiNeRF) & $\overbar{R'_t}$ & $\overbar{R_t}$ & $|\overbar{R'_t}$ - $\overbar{R_t}|$ \\
 \includegraphics[width=25mm]{Figures/figure_inter/rgb00_fern.png}&\includegraphics[width=25mm]{Figures/figure_inter/rgb0_fern.png}&\includegraphics[width=25mm]{Figures/figure_inter/rgb0_grad_fern.png}&\includegraphics[width=25mm]{Figures/figure_inter/fern.png}
 &\includegraphics[width=25mm]{Figures/figure_inter/depth00_fern.png}
 &\includegraphics[width=25mm]{Figures/figure_inter/depth0_fern.png}&\includegraphics[width=25mm]{Figures/figure_inter/depthdiff_fern.png} \\
  % \includegraphics[width=25mm]{Figures/figure_inter/rgb00_horns.png}&\includegraphics[width=25mm]{Figures/figure_inter/rgb0_horns.png}&\includegraphics[width=25mm]{Figures/figure_inter/rgb0_grad_horns.png}&\includegraphics[width=25mm]{Figures/figure_inter/horns.png}
  % &\includegraphics[width=25mm]{Figures/figure_inter/depth00_horns.png}
 % &\includegraphics[width=25mm]{Figures/figure_inter/depth0_horns.png}&\includegraphics[width=25mm]{Figures/figure_inter/depthdiff_horns.png} \\
  \includegraphics[width=25mm]{Figures/figure_inter/rgb00_trex.png}&\includegraphics[width=25mm]{Figures/figure_inter/rgb0_trex.png}&\includegraphics[width=25mm]{Figures/figure_inter/rgb0_grad_trex.png}&\includegraphics[width=25mm]{Figures/figure_inter/trex.png}
&\includegraphics[width=25mm]{Figures/figure_inter/depth00_trex.png}
 &\includegraphics[width=25mm]
 {Figures/figure_inter/depth0_trex.png}&\includegraphics[width=25mm]{Figures/figure_inter/depthdiff_trex.png}\\
\end{tblr}

==> Figures/figure_llff_avr.tex <==
\begin{tblr}{
  stretch = 0,
  colsep  = 0pt,
  colspec = {Q[h,c]Q[h,c]Q[h,c]},
  rowsep = 0.3pt,
}
  \small{Ground Truth} & \small{PAS-8 $\bm{c}_f$ (AVR)} & \small{PAS-8 $\bm{c}_f$ (Reg)}\\
  \includegraphics[width=60mm]{Figures/figure_avr/horns_gt.jpg} &\includegraphics[width=60mm]{Figures/figure_avr/horns_avr.jpg}&\includegraphics[width=60mm]{Figures/figure_avr/horns_reg.jpg} \\
    \includegraphics[width=60mm]{Figures/figure_avr/orchids_gt.jpg} &\includegraphics[width=60mm]{Figures/figure_avr/orchids_avr.jpg}&\includegraphics[width=60mm]{Figures/figure_avr/orchids_reg.jpg} \\
      \includegraphics[width=60mm]{Figures/figure_avr/trex_gt.jpg} &\includegraphics[width=60mm]{Figures/figure_avr/trex_avr.jpg}&\includegraphics[width=60mm]{Figures/figure_avr/trex_reg.jpg} \\
        \includegraphics[width=60mm]{Figures/figure_avr/room_gt.jpg} &\includegraphics[width=60mm]{Figures/figure_avr/room_avr.jpg}&\includegraphics[width=60mm]{Figures/figure_avr/room_reg.jpg} \\
\end{tblr}

==> Figures/figure_nt.tex <==
\begin{tblr}{
  stretch = 0,
  colsep  = 0pt,
  colspec = {Q[h,c]Q[h,c]Q[h,c]},
  rowsep = 1pt,
}
  \small{Ground Truth} & \small{NeRF} & \small{$N_t=17$ (full)} \\
  
  \includegraphics[width=57mm]{Figures/Figure_Nt/001_gtv.png} &
  \includegraphics[width=57mm]{Figures/Figure_Nt/001_nerf.png} &
  \includegraphics[width=57mm]{Figures/Figure_Nt/001_17v.png} \\ 
  
  \small{$N_t=12$} & \small{$N_t=8$} & \small{$N_t=5$} \\
  \includegraphics[width=57mm]{Figures/Figure_Nt/001_12v.png} & 
  \includegraphics[width=57mm]{Figures/Figure_Nt/001_8v.png} & 
  \includegraphics[width=57mm]{Figures/Figure_Nt/001_5v.png}\\
  
\end{tblr}

==> Figures/figure_pas_distribution.tex <==
\begin{tblr}{
  stretch = 0,
  colsep  = 3pt,
  colspec = {Q[c,c]Q[h,c]},
  rowsep = 0.3pt,
}
  Dense $\sigma$ values &\includegraphics[width=150mm]{Figures/figure_ablation_affine/dense_sigma.png} \\
  Dense $\alpha$ values &\includegraphics[width=150mm]{Figures/figure_ablation_affine/dense_alpha.png}\\
  Sparse $\alpha$ values&\includegraphics[width=150mm]{Figures/figure_ablation_affine/sparse_alpha.png} \\
  PAS-VRE $\hat{\alpha}$ values &\includegraphics[width=150mm]{Figures/figure_ablation_affine/affine_sparse_alpha.png} \\
\end{tblr}

==> Figures/figure_pas_vre.tex <==
\begin{tblr}{
  stretch = 0,
  colsep  = 0pt,
  colspec = {Q[h,c]Q[h,c]Q[h,c]},
  rowsep = 0.3pt,
}
  \small{Dense Sampling} & \small{Sparse Sampling + VRE} & \small{Sparse Sampling + PAS-VRE} \\
  \includegraphics[width=60mm]{Figures/figure_ablation_affine/img_full.jpg} &\includegraphics[width=60mm]{Figures/figure_ablation_affine/img_no_Affine.jpg}&\includegraphics[width=60mm]{Figures/figure_ablation_affine/img_affine.jpg} \\
  \includegraphics[width=60mm]{Figures/figure_ablation_affine/depth_full.jpg} &\includegraphics[width=60mm]{Figures/figure_ablation_affine/depth_no_Affine.jpg}&\includegraphics[width=60mm]{Figures/figure_ablation_affine/depth_affine.jpg} \\
\end{tblr}

==> Figures/figure_points_offset.tex <==
\begin{tblr}{
  stretch = 0,
  colsep  = 0pt,
  colspec = {Q[h,c]Q[h,c]Q[h,c]Q[h,c]},
  rowsep = 0.3pt,
}
  \small{Ground Truth} & \small{With points offset} & \small{W/o points offset} & \small{Offset magnitude heatmap}\\
  \includegraphics[width=44mm]{Figures/figure_points_offset/box_gt.png} &\includegraphics[width=44mm]{Figures/figure_points_offset/box_correct.png}&\includegraphics[width=44mm]{Figures/figure_points_offset/box_wrong.png} &\includegraphics[width=44mm]{Figures/figure_points_offset/box_mask.png}\\
  \includegraphics[width=44mm]{Figures/figure_points_offset/box_gt_2.png} &\includegraphics[width=44mm]{Figures/figure_points_offset/box_correct_2.png}&\includegraphics[width=44mm]{Figures/figure_points_offset/box_wrong_2.png} &\includegraphics[width=44mm]{Figures/figure_points_offset/box_mask_2.png}\\
  \includegraphics[width=44mm]{Figures/figure_points_offset/box_gt_3.png} &\includegraphics[width=44mm]{Figures/figure_points_offset/box_correct_3.png}&\includegraphics[width=44mm]{Figures/figure_points_offset/box_wrong_3.png} &\includegraphics[width=44mm]{Figures/figure_points_offset/box_mask_3.png}\\
\end{tblr}

==> Figures/figure_pseudo_data.tex <==
\begin{tblr}{
  stretch = 0,
  colsep  = 0pt,
  colspec = {Q[h,c]Q[h,c]Q[h,c]},
  rowsep = 0.3pt,
}
$\hat{\bm{c}}_f$ & $\hat{\bm{c}}(\bm{r})$ & Uncertainty ground truth\\
  \includegraphics[width=60mm]{Figures/figure_pseudo_data/fortress_000_avr.png} &\includegraphics[width=60mm]{Figures/figure_pseudo_data/fortress_000_nerf.png}&\includegraphics[width=60mm]{Figures/figure_pseudo_data/fortress_000_mask.png} \\
  \includegraphics[width=60mm]{Figures/figure_pseudo_data/trex_000_avr.png} &\includegraphics[width=60mm]{Figures/figure_pseudo_data/trex_000_nerf.png}&\includegraphics[width=60mm]{Figures/figure_pseudo_data/trex_000_mask.png} \\
    \includegraphics[width=60mm]{Figures/figure_pseudo_data/room_000_avr.png} &\includegraphics[width=60mm]{Figures/figure_pseudo_data/room_000_nerf.png}&\includegraphics[width=60mm]{Figures/figure_pseudo_data/room_000_mask.png} \\
\end{tblr}

==> Figures/figure_ref_views.tex <==
\begin{tblr}{
  stretch = 0,
  colsep  = 0pt,
  colspec = {Q[h,c]Q[h,c]},
  rowsep = 0.3pt,
}
  \small{Fortress} & \small{Fern} \\
  \includegraphics[width=44mm]{Figures/figure_ref_views/fortress_cam.JPG} &\includegraphics[width=44mm]{Figures/figure_ref_views/fern_cam.JPG}\\
\end{tblr}

==> Figures/figure_splash_2.tex <==
 \begin{tblr}{
  stretch = 0,
  colsep  = 0pt,
  rowsep  = 0.3pt,
  colspec = {Q[h,c]Q[h,c]Q[h,c]},
}
  \small{Ground Truth} & \small{EpiNeRF-12 (Ours)} & \small{NeRF-192} \cite{nerf}\\
    {\includegraphics[width=27mm]{Figures/figure_splash/fern_patch_gt.jpg}} & {\includegraphics[width=27mm]{Figures/figure_splash/fern_patch_our.jpg}}& {\includegraphics[width=27mm]{Figures/figure_splash/fern_patch_nerf.jpg}} \\

    {\includegraphics[width=27mm]{Figures/figure_splash/horns_patch_gt.jpg}} & {\includegraphics[width=27mm]{Figures/figure_splash/horns_patch_our.jpg}}& {\includegraphics[width=27mm]{Figures/figure_splash/horns_patch_nerf.jpg}} \\ 

       {\includegraphics[width=27mm]{Figures/figure_splash/flower_patch_gt.jpg}} & {\includegraphics[width=27mm]{Figures/figure_splash/flower_patch_our.jpg}}& {\includegraphics[width=27mm]{Figures/figure_splash/flower_patch_nerf.jpg}} \\



\end{tblr}

% merge figure 1 and 2 to one figure

==> Tables/table_ablation_Nn_Nt.tex <==
% \begin{tabular}{lccccccc}
% \hline
% Scene & $N_s$ & $N_t$ & $N_n$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\ 
% \hline
% Fern & 12 & 5 & 4 & 22.250 & 0.705 & 0.339 \\
% Fern & 12 & 8 & 4 & 24.149 & 0.778 & 0.274 \\
% Fern & 12 & 12 & 4 & 24.444 & 0.790 & 0.261 \\
% \hline
% Fern & 12 & 17 & 2 & 24.709 & 0.792 & 0.253 \\
% Fern & 12 & 17 & 3 & 24.899 & 0.799 & 0.252 \\
% Fern & 12 & 17 & 5 & 25.043 & {0.802} & 0.256 \\
% Fern & 12 & 17 & 6 & 24.486 & 0.789 & 0.256 \\
% Fern & 12 & 17 & 8 & 24.723 & 0.790 & 0.262 \\
% % 12 & 17 & 10 & 25.258 & 0.808 & 0.251 \\
% \hline
% Fern (undistorted) & 12 & 17 & 4 & 25.078 & \textbf{0.809} & \textbf{0.238} \\
% \hline
% Fern & 12 & 17 & 4 & \textbf{25.170} & 0.807 & 
% 0.244 \\
% \hline

% \end{tabular}

\begin{tabular}{lccccc}
\hline
Scene  & $N_n$ & PSNR\cellcolor{c_highbest} & SSIM\cellcolor{c_highbest} & LPIPS\cellcolor{c_lowbest} \\ 
\hline
Fern  & 2 & 24.709 & 0.792 & 0.253 \\
Fern  & 3 & 24.899 & 0.799 & 0.252 \\
Fern  & 5 & 25.043 & {0.802} & 0.256 \\
Fern  & 6 & 24.486 & 0.789 & 0.256 \\
Fern  & 8 & 24.723 & 0.790 & 0.262 \\
% \hline
% Fern (undistorted) & 4 & 25.078 & \textbf{0.809} & \textbf{0.238} \\
\hline
Fern & 4 & \textbf{25.170} & 0.807 & 0.244 \\
\hline

\end{tabular}

==> Tables/table_blender.tex <==
\begin{tabular}{lccccc}
\hline
 Methods  & PSNR\cellcolor{c_highbest} & SSIM$_{t}$\cellcolor{c_highbest} & LPIPS$_{vgg}$\cellcolor{c_lowbest} & FPS\cellcolor{c_highbest} & Mem(MB)\cellcolor{c_lowbest} \\ 
\hline

NeRF (ECCV20) & 31.00 & 0.947 & 0.081 & 0.36  & 5.0 \\
SNeRG (ICCV21)  & 30.38 & 0.950 & 0.050 & \textbf{202} & 84.0 \\
Plenoxels (CVPR22)   & 31.71 & 0.958 & 0.049 & 10.8 & 3000 \\
TensoRF-CP (ECCV22) & 31,56 &  0.949 & 0.076 & 0.45 & \textbf{3.9} \\
TensoRF-VM (ECCV22) & 33.14 &  0.963 & 0.047& 0.38 & 71.8 \\
INGP (SIGGRAPH22) & \textbf{33.18} & \textbf{0.974} & \textbf{0.043} & 8.7 & 27.0 \\
\cdashline{1-6}
ProNeRF-32 Prune & 31.92 & 0.959 & 0.056 & 3.2 &  6.3 \\
ProNeRF-32 & 31.95 & 0.959 & 0.057 & 1.2 &  5.2 \\
\hline
\end{tabular}

==> Tables/table_blender_hyperreel.tex <==
\begin{tabular}{lccccccccc}
Methods & Chair & Drums & Ficus & Hotdog & Lego  & Materials & Mic & Ship & Average\\ 
\hline
Hyperreel & 21.48 & 16.16 & 19.42 & 26.20 & 17.67  & 15.62 & 21.91 & 19.31 & \textbf{19.72}\\
\hline
\end{tabular}

==> Tables/table_blender_scene.tex <==
\begin{tabular}{lccccccccc}
\multicolumn{10}{c}{PSNR$\uparrow$}\\
\hline
Methods & Chair & Drums & Ficus & Hotdog & Lego  & Materials & Mic & Ship & Average\\ 
\hline
ProNeRF-32 Prune & 34.52 & 24.76 & 31.22 & 37.69 & 33.19  & 30.59 & 33.85 & 29.48 & 31.92\\
ProNeRF-32 & 34.57 & 24.77 & 31.28 & 37.69 & 33.19  & 30.59 & 34.00 & 29.48 & 31.95\\
\hline

\\
\multicolumn{10}{c}{SSIM$_t$$\uparrow$}\\
\hline
Methods & Room & Fern & Leaves & Fortress & Orchids  & Flower & T-Rex & Horns& Average\\ 
\hline
% NeRF \cite{nerf} & 0.948 & 0.793 & 0.690 & 0.881 & 0.641  & 0.827 & 0.880 & 0.828 & 0.811 \\
% \hline

ProNeRF-32 Prune & 0.983 & 0.926 & 0.973 & 0.985 & 0.971  & 0.960 & 0.987 & 0.887 & 0.959\\
ProNeRF-32 & 0.983 & 0.926 & 0.973 & 0.985 & 0.971  & 0.960 & 0.987 & 0.887 & 0.959\\
\hline
\\
\multicolumn{10}{c}{LPIPS$_{vgg}$$\uparrow$}\\
\hline
Methods & Room & Fern & Leaves & Fortress & Orchids  & Flower & T-Rex & Horns& Average\\ 
\hline
% NeRF \cite{nerf} & 0.948 & 0.793 & 0.690 & 0.881 & 0.641  & 0.827 & 0.880 & 0.828 & 0.811 \\
% \hline
ProNeRF-32 Prune & 0.023 & 0.093 & 0.034 & 0.029 & 0.038  & 0.057 & 0.015 & 0.161 & 0.056\\
ProNeRF-32 & 0.024 & 0.094 & 0.033 & 0.029 & 0.039  & 0.057 & 0.016 & 0.161 & 0.057\\
\hline
\end{tabular}

==> Tables/table_blender_time_rebuttal.tex <==
\begin{tabular}{lccccccccc}
Methods & Chair & Drums & Ficus & Hotdog & Lego  & Materials & Mic & Ship & Average\\ 
\hline
ProNeRF-32 Prune & 4.7 & 2.4 & 4.7 & 2.4 & 2.4  & 2.4 & 4.7 & 2 & \textbf{3.2}\\
\hline
\end{tabular}

==> Tables/table_donerf.tex <==
\begin{tabular}{lccc}
\hline
Method & PSNR$\uparrow$  & FPS$\uparrow$ & Memory (MB) $\downarrow$\\ 

{NeRF } & {{30.9}} & {0.4} & \textbf{3.8} \\

\multirow{2}{*}{DONeRF }  &  29.8 & 6.4 & 4.1 \\
   &  30.9 & 3.4 & 4.1 \\


 \multirow{2}{*}{TermiNeRF }   &  29.2 & 6.4 & 4.1 \\
   &  29.8 & 3.4 & 4.1 \\

\multirow{2}{*}{AdaNeRF }   & 29.5 & \textbf{12.7} & 4.1 \\
  & 30.8 & 7.7 & 4.1 \\
\hline
{Ours} & {\textbf{33.2}} & {8.2} & {{4.7}}\\
\hline
\end{tabular}

==> Tables/table_llff_rebuttal.tex <==
\begin{tabular}{lccccccc}
\hline
Method & Type &PSNR & SSIM & LPIPS & FPS  & MB\\
\hline
NeRF  & \textbf{R} & 26.50 &  \cellcolor{bot2}0.811$_{t}$ &  \cellcolor{bot2}0.250$_{v}$ & 0.3  & \cellcolor{top2}3.8 \\
MipNeRF (H)  & \textbf{R}  & 27.01 & \cellcolor{top3}0.845$_{t}$ & 0.148$_{u}$ &  \cellcolor{bot3}0.03 & 5.7 \\
MipNeRF 360 (H) & \textbf{R} & 26.86 & \cellcolor{top2}0.858$_{t}$ & 0.128$_{u}$ &  \cellcolor{bot5}0.1 &  8.2 \\
Instant NGP  & \textbf{RD}  &  25.60 &   \cellcolor{bot1}0.758$_{t}$ &  \cellcolor{bot1}0.267$_{v}$ & 7.3 & 64.0 \\
Plenoxels  & \textbf{RD}  & 26.30 &  0.839$_{t}$ & 0.210$_{v}$ & 9.1 &  \cellcolor{bot2}3629.8 \\
TensoRF  & \textbf{RD}  & 26.73 & 0.839$_{t}$ & \cellcolor{top2}0.204$_{v}$ & 1.1 & 179.7 \\
MobileNeRF  & \textbf{RD} & 25.91 & 0.825$_{t}$ & 0.183$_{u}$ & \cellcolor{top2}349 &  \cellcolor{bot5}201.50 \\
SNeRG  & \textbf{RDP} &  25.63 & \cellcolor{bot3}0.818$_{t}$ & 0.183$_{u}$ & 50.7\cellcolor{top5} &  \cellcolor{bot4}337.25 \\
EfficientNeRF  & \textbf{RDP} & \cellcolor{top1}27.39 & \cellcolor{top1}0.912$_{s}$ & 0.082$_{u}$ & 219 \cellcolor{top4} &  \cellcolor{bot3}2800 \\
ENeRF  & \textbf{RE} & \cellcolor{bot3}24.89 &  0.865$_{s}$ & \cellcolor{top1}0.159$_{v}$ & 8.9  & \cellcolor{top1}2.9 \\
FastNeRF(cache)*  & \textbf{RDP} & 26.04 \cellcolor{bot1}& 0.856$_{s}$ \cellcolor{bot1}& 0.085$_{a}$ \cellcolor{bot1}& \cellcolor{top1}700 &  \cellcolor{bot1}4100 \\
RSEN*  & \textbf{R} & \cellcolor{bot2}27.45 & \cellcolor{bot2}0.905$_{s}$ & \cellcolor{top2}0.060$_{a}$ & 0.34 &  5.4 \\
R2L*  & \textbf{RP} & 27.79 & 0.973$_{s}$ \cellcolor{top1}& 0.097$_{a}$ \cellcolor{bot2}& 5.6 &  22.6 \\
% DONeRF & \textbf{S}  & 22.9 & - & - & 2.8 &  4.1 \\
% TermiNeRF & \textbf{S}  & 23.6 & - & - & 2.8 &  4.1\\
% AdaNeRF  & \textbf{S} & 25.7 & - & - & 7.7 &  4.1 \\
% IBRNet$\dagger$  & \textbf{L} & 26.73 & 0.851 & 0.175$_{v}$ & 0.06 &  34.2 \\
% NeX$\dagger$  & \textbf{L} & 27.26 & 0.904 & 0.178$_{v}$ & 300 &  88.8 \\
% NLF$\dagger$  & \textbf{L} & 28.26 & 0.920 & 0.062$_{v}$ & 0.002 &  25 \\

% \hline

% EpiNeRF-12 & \textbf{S} & {27.15} & {0.837} & {0.216} & 4.4 &  4.7 \\
% EpiNeRF-12 (large) & \textbf{S} & 27.28 & 0.838 & 0.208 & 3.5 &  5.5 \\
% EpiNeRF-12 (large)$\dagger$ & \textbf{S} & 27.38 & 0.846 & 0.201 & 3.5 &  5.5 \\
% EpiNeRF-8* & \textbf{S} & 0 & 0 & 0 & 0 &  0 \\
% EpiNeRF-12* & \textbf{S} & 28.33 & 0.885 & 0.129 & 4.4 &  4.7 \\

\hline

\end{tabular}

==> Tables/table_llff_rebuttal_b.tex <==
\begin{tabular}{lccccccc}
\hline
Method & Type & PSNR & SSIM & LPIPS & FPS  & MB\\ 
\hline
% NeRF  & \textbf{R} & 26.50 & 0.811 & 0.250$_{v}$ & 0.3  & 3.8 \\
% Jax Mip-NeRF (512 hiddens)  & \textbf{R}  & 27.01 & 0.845 & 0.148$_{u}$ & 0.03 & 5.7 \\
% Jax Mip-NeRF 360 (512 hiddens)  & \textbf{R} & 26.86 & 0.858 & 0.128$_{u}$ & 0.1 &  8.2 \\
% Instant NGP  & \textbf{D}  & 25.60 &  0.758 & 0.267$_{v}$ & 7.3 & 64.0 \\
% Plenoxels  & \textbf{D}  & 26.30 &  0.839 & 0.210$_{v}$ & 9.1 & 3629.8 \\
% TensoRF  & \textbf{D}  & 26.73 & 0.839 & 0.204$_{v}$ & 1.1 & 179.7 \\
% MobileNeRF  & \textbf{D} & 25.91 & 0.825 & 0.183$_{u}$ & 349.34 &  201.50 \\
% SNeRG  & \textbf{P} & 25.63 & 0.818 & 0.183$_{u}$ & 50.7 &  337.25 \\
% EfficientNeRF  & \textbf{P} & 27.39 & 0.912 & 0.082$_{u}$ & 218.8 &  2800 \\
% FastNeRF (cache)*  & \textbf{P} & 26.04 & 0.856 & 0.085$_{u}$ & 700 &  4100 \\
% R2L*  & \textbf{P} & 27.79 & 0.973 & 0.097$_{a}$ & 5.6 &  22.6 \\
DONeRF & \textbf{RPS}  & \cellcolor{bot1}22.9 & - & - & 2.8 &  \cellcolor{top3}4.1 \\
TermiNeRF & \textbf{RPS}  & \cellcolor{bot2}23.6 & - & - & 2.8 &  \cellcolor{top3}4.1\\
AdaNeRF  & \textbf{RS} & 25.7 & - & - & 7.7 &  \cellcolor{top3}4.1 \\
IBRNet$\dagger$  & \textbf{RE} &  \cellcolor{bot1}26.73 &  \cellcolor{bot2}0.851$_{t}$ & \cellcolor{bot3}0.175$_{v}$ &  \cellcolor{bot4}0.06 &   34.2 \\
NeX$\dagger$  & \textbf{RD} &  \cellcolor{bot3}27.26 & \cellcolor{top3}0.904$_{s}$ &  \cellcolor{bot2}0.178$_{v}$ & \cellcolor{top3}300 &   88.8 \\
NeuRay$\dagger$  & \textbf{RE} & \cellcolor{bot2}27.06 & \cellcolor{bot1}0.850$_{t}$ & \cellcolor{top3}0.172$_{v}$ & 2.3 &  12.0 \\
GPNR$\dagger$  & \textbf{RE} & 27.66\cellcolor{top2}&\cellcolor{top1} 0.924$_{s}$ & \cellcolor{top2}0.138$_{v}$ & \cellcolor{bot1}0.001 & 37  \\
NLF$\dagger$  & \textbf{RE} & \cellcolor{top1}28.26 & \cellcolor{top2}0.920$_{s}$ & \cellcolor{top1}0.062$_{v}$ &  \cellcolor{bot2}0.002 &  25 \\

\hline

Our-12 & \textbf{RSE} & \cellcolor{top3}{27.15} & {0.894}$_{s}$,{0.837}$_{t}$ & {0.216}$_{v}$ & 4.4 &  4.7 \cellcolor{top4}\\
Our-12 (H) & \textbf{RSE} & \cellcolor{top2}27.28 & {0.894}$_{s}$,0.838$_{t}$ & 0.208$_{v}$ & 3.8 &  \cellcolor{top5}5.0 \\
Our-12 (H)$\dagger$ & \textbf{RSE} & \cellcolor{top3}27.38 &  \cellcolor{bot3}0.902$_{s}$,0.850$_{t}$ &  \cellcolor{bot1}0.199$_{v}$ & 3.8 &  \cellcolor{top5}5.0 \\
Our-8* & \textbf{RSE} & 28.08\cellcolor{top2} & 0.916$_{s}$, 0.879$_{t}$ & 0.060$_{a}$ \cellcolor{top2}&  6.9&  4.7 \cellcolor{top4}\\
Our-12* & \textbf{RSE} & 28.33\cellcolor{top1} & 0.920\cellcolor{top2}$_{s}$, 0.885$_{t}$ & 0.058$_{a}$ \cellcolor{top1}& 4.4 &  4.7 \cellcolor{top4}\\

\hline

\end{tabular}

==> Tables/table_llff_scene.tex <==
\begin{tabular}{lccccccccc}
\multicolumn{10}{c}{PSNR$\uparrow$}\\
\hline
Methods & Room & Fern & Leaves & Fortress & Orchids  & Flower & T-Rex & Horns & Average\\ 
\hline
% NeRF \cite{nerf} & \textbf{32.70} & \textbf{25.17} & 20.92 & 31.16 & 20.36  & 27.40 & 26.80 & 27.45 & 26.50 \\
% \hline
% DONeRF \cite{donerf} & 27.06 & 21.62 & 17.68 & 27.46 & 18.04  & 23.78 & 23.52 & 24.08 & 22.91 \\
% TermiNeRF \cite{terminerf} & 27.70 & 23.24 & 17.89 &  27.58 & 17.87  & 24.27 &  24.81 & 25.04 & 23.55 \\
% AdaNeRF \cite{adanerf} & 31.23 & 23.39 & 20.53 & 30.44 & 19.64  & 27.57 & 26.03 & 26.86 & 25.71 \\
% \hline
ProNeRF-8 Prune & 32.13 & 25.00 & 21.07 & 31.29 & 19.85  & 27.96 & 26.96 & 28.06 & 26.54\\
ProNeRF-8 & 32.20 & 25.04 & 21.17 & 31.93 & 20.06  & 28.32 & 27.11 & 28.37 & 26.78\\
ProNeRF-12 & 32.44 & 25.17 & 22.09 & 31.90 & 20.64  & 28.52 & 27.73 & 28.71 & 27.15\\
\hline
\\
\multicolumn{10}{c}{SSIM$_t$$\uparrow$}\\
\hline
Methods & Room & Fern & Leaves & Fortress & Orchids  & Flower & T-Rex & Horns& Average\\ 
\hline
% NeRF \cite{nerf} & 0.948 & 0.793 & 0.690 & 0.881 & 0.641  & 0.827 & 0.880 & 0.828 & 0.811 \\
% \hline

ProNeRF-8 Prune & 0.946 & 0.811 & 0.730 & 0.894 & 0.620  & 0.851 & 0.892 & 0.858 & 0.825\\
ProNeRF-8 & 0.946 & 0.808 & 0.710 & 0.907 & 0.630  & 0.851 & 0.890 & 0.854 & 0.825\\
ProNeRF-12 & 0.949 & 0.809 & 0.757 & 0.906 & 0.658  & 0.857 & 0.904 & 0.860 & 0.838\\
\hline
\\
\multicolumn{10}{c}{SSIM$_s$$\uparrow$}\\
\hline
Methods & Room & Fern & Leaves & Fortress & Orchids  & Flower & T-Rex & Horns& Average\\ 
\hline
% NeRF \cite{nerf} & 0.948 & 0.793 & 0.690 & 0.881 & 0.641  & 0.827 & 0.880 & 0.828 & 0.811 \\
% \hline
ProNeRF-8 Prune & 0.972 & 0.870 & 0.795 & 0.944 & 0.723  & 0.914 & 0.929 & 0.919 & 0.883\\
ProNeRF-8 & 0.973 & 0.870 & 0.785 & 0.950 & 0.732  & 0.914 & 0.930 & 0.919 & 0.884\\
ProNeRF-12 & 0.974 & 0.871 & 0.821 & 0.950 & 0.756  & 0.919 & 0.939 & 0.923 & 0.894\\
\hline
\\
\multicolumn{10}{c}{LPIPS$_{vgg}$$\downarrow$}\\
\hline
Methods & Room & Fern & Leaves & Fortress & Orchids  & Flower & T-Rex & Horns& Average\\ 
\hline
% NeRF \cite{nerf} & 0.178 & 0.280 & 0.316 & 0.171 & 0.321  & 0.219 & 0.249 & 0.268 & 0.250\\
% \hline
ProNeRF-8 Prune & 0.174 & 0.238 & 0.255 & 0.155 & 0.297  & 0.174 & 0.228 & 0.228 & 0.219\\
ProNeRF-8 & 0.176 & 0.250 & 0.295 & 0.143 & 0.305  & 0.177 & 0.232 & 0.244 & 0.228\\
ProNeRF-12 & 0.173 & 0.244 & 0.258 & 0.153 & 0.284  & 0.171 & 0.212 & 0.237 & 0.216\\
\hline
\\
\multicolumn{10}{c}{LPIPS$_{alex}$$\downarrow$}\\
\hline
Methods & Room & Fern & Leaves & Fortress & Orchids  & Flower & T-Rex & Horns& Average\\ 
\hline
% NeRF \cite{nerf} & 0.178 & 0.280 & 0.316 & 0.171 & 0.321  & 0.219 & 0.249 & 0.268 & 0.250\\
% \hline
ProNeRF-8 Prune & 0.079 & 0.138 & 0.160 & 0.074 & 0.193  & 0.093 & 0.089 & 0.130 & 0.120\\
ProNeRF-8 & 0.083 & 0.145 & 0.161 & 0.061 & 0.188  & 0.089 & 0.085 & 0.140 & 0.119\\
ProNeRF-12 & 0.082 & 0.136 & 0.128 & 0.064 & 0.169  & 0.086 & 0.071 & 0.136 & 0.109\\
\hline
\end{tabular}

==> Tables/table_llff_undistort.tex <==
\begin{tabular}{clccccc}
\hline
Res. & Methods  & PSNR\cellcolor{c_highbest} & SSIM$_{t/s}$\cellcolor{c_highbest} & LPIPS$_{vgg/alex}$\cellcolor{c_lowbest} & FPS\cellcolor{c_highbest} & Mem(MB)\cellcolor{c_lowbest} \\ 
\hline

 & NeRF (ECCV20) & 26.50 & 0.811 / - & 0.250 / - & 0.3  & 3.8 \\
&INGP (SIGGRAPH22)   & 25.60 & 0.758 / - & 0.267 / - & 7.3 & 64.0 \\
\multirow{9}{*}{$756$}&Plenoxels (CVPR22) & 26.30 &  0.839 / - & 0.210 / - & 9.1 & 3629.8 \\
\multirow{9}{*}{$ \times $}& MipNeRF360 (CVPR22) & 26.86 & \textbf{0.858} / - & - / 0.128 &  0.1 &  8.2 \\
\multirow{9}{*}{$1008$}&TensoRF (ECCV22)   & 26.73 & 0.839 / - & 0.204 / 0.124 & 1.1 & 179.7 \\
&K-Planes (CVPR23)  & 26.92 &  {0.847} / - & 0.182 / - & 0.7 & 214 \\
&SNeRG (ICCV21)  & 25.63 & 0.818 / - & 0.183 / - & 50.7 & 337.3 \\
% &EfficientNeRF   & 27.39 & 0.912 & 0.082 & 219 & 2800 \\
% &DONeRF  & 22.9 & - & - & 2.8 &  4.1 \\
&ENeRF (SGGRPHA22) & 24.89 & - / 0.865 & \textbf{0.159} / - & 8.9 &  10.7\\
&AdaNeRF (ECCV22) & 25.70 & - / - & - / - & 7.7 &  4.1 \\
&Hyperreel (CVPR23) & 26.20 & - / - & - / - & 4.0 & 58.8 \\
&MobileNeRF (CVPR23) & 25.91 & 0.825 / - & 0.183 / - & \textbf{348} & 201.5 \\

\cdashline{2-7}

% &ProNeRF-0($C_{s_1}$) & 24.83 & 0.787 / - & 0.236 & 29.4  &  3.1 \\
% &ProNeRF-4 & 25.61 & 0.791 & 0.248 & 12.5  &  4.7 \\
&PAS-8 $\bm{c}_{f}$ (Reg) (Ours) & 24.86 & 0.787 / 0.855 & 0.236 / 0.150 & 29.4 &  \textbf{2.7}  \\
&PAS-8 $\bm{c}_{f}$ (AVR) (Ours) & 25.15 & 0.793 / 0.860 & 0.234 / 0.146 & 25.6 &  5.0  \\
&ProNeRF-8 Prune (Ours)& 26.54 & 0.825 / 0.883 & 0.219 / 0.120 & 8.5 &  6.8 \\
&ProNeRF-8 (Ours)  & 26.78 & 0.825 / 0.884 & 0.228 / 0.119 & 6.9 &  3.5 \\
&ProNeRF-12 (Ours) & \textbf{27.15} & 0.838 / \textbf{0.894} & 0.217 / \textbf{0.109} & 4.4 &  3.5 \\
\hline

 & NeRF (ECCV20) & 26.76 & - / 0.883 & 0.246 / - & 0.3  & 3.8 \\
\multirow{3}{*}{Undist} & IBRNet (CVPR21) & 26.73 & - / 0.851 & 0.175 / - & 0.06  & 34.2 \\
\multirow{3}{*}{$756 $}&NeX (CVPR21)  & 27.26 & - / 0.904 & 0.178 / - & \textbf{300} & 88.8 \\
\multirow{3}{*}{$ \times $}&NeuRay (CVPR22)   & 27.06 & - / 0.859 & 0.172 / - & 2.3 & 12.0 \\
\multirow{3}{*}{$ 1008$}&GPNR (ECCV22) & 27.66 &  - / \textbf{0.924} & 0.138 / - & 0.001 & 37.0 \\
&LFNR (CVPR22) & \textbf{28.26} & - / 0.920 & \textbf{0.127} / - & 0.002 & 25.0 \\
\cdashline{2-7}
&ProNeRF-12 & 27.38 & 0.849 / 0.902 & 0.199 / 0.099 & {4.4} &  \textbf{3.5} \\
\hline
\end{tabular}
